BiCro: Noisy Correspondence Rectification for Multi-modality Data via Bi-directional Cross-modal Similarity Consistency

As one of the most fundamental techniques in multimodal learning, cross-modal matching aims to project various sensory modalities into a shared feature space. To achieve this, massive and correctly aligned data pairs are required for model training. However, unlike unimodal datasets, multimodal datasets are extremely harder to collect and annotate precisely. As an alternative, the co-occurred data pairs (e.g., image-text pairs) collected from the Internet have been widely exploited in the area. Unfortunately, the cheaply collected dataset unavoidably contains many mismatched data pairs, which have been proven to be harmful to the model's performance. To address this, we propose a general framework called BiCro (Bidirectional Cross-modal similarity consistency), which can be easily integrated into existing cross-modal matching models and improve their robustness against noisy data. Specifically, BiCro aims to estimate soft labels for noisy data pairs to reflect their true correspondence degree. The basic idea of BiCro is motivated by that -- taking image-text matching as an example -- similar images should have similar textual descriptions and vice versa. Then the consistency of these two similarities can be recast as the estimated soft labels to train the matching model. The experiments on three popular cross-modal matching datasets demonstrate that our method significantly improves the noise-robustness of various matching models, and surpass the state-of-the-art by a clear margin.

==> CVPR23__Cross-modal_Noise-2/algo.tex <==
\begin{algorithm*}[th!]
\KwIn{A noisily-labeled dataset $\tilde{\mathcal{D}}$}
{
\textbf{Required}: the clean probability threshold $\delta$, two individual matching models $A$ and $B$ with different initializations and data batch sequences}

Warm up the model $(A,B)$ using $L_{hard}$ Eq.~\ref{eq:triplet_loss}.

\For{$i=1:num\_epochs$}
{
\textcolor{blue}{//Section.~\ref{sec:anchor_point}: modeling per-sample loss distribution using Eq.~\ref{eq:clean_posterior}}

$\mathcal{P}^A = \{p_i^A \mid p_i^A = p\left(k=0 \mid \ell_i\right)\}_{i=1}^N \leftarrow BetaMixtureModel(\tilde{\mathcal{D}},B)$

$\mathcal{P}^B = \{p_i^B \mid p_i^B = p\left(k=0 \mid \ell_i\right)\}_{i=1}^N \leftarrow BetaMixtureModel(\tilde{\mathcal{D}},A)$

\For{$k \in \{A,B\}$}
{
$\Tilde{\mathcal{D}}^k_c = \{(I_i,T_i,y_i=1) \mid p_i^k > \delta, \forall (I_i,T_i) \in \Tilde{\mathcal{D}}\}$ \hfill \textcolor{blue}{//Section.~\ref{sec:anchor_point}: anchor points selection using Eq.~\ref{eq:anchor_select}}

$\Tilde{\mathcal{D}}^k_n = \{(I_i,T_i) \mid p_i^k \leq \delta, \forall (I_i,T_i) \in \Tilde{\mathcal{D}}\}$\hfill \textcolor{blue}{//Section.~\ref{sec:anchor_point}: noisy data selection using Eq.~\ref{eq:noisy_select}}


\For{$j=1:num\_steps$}
{
Sample a mini-batch $\{\mathcal{B}_j^c = (I_c,T_c,y_c=1), \mathcal{B}_j^n= (I_n,T_n)\}$ from $\{\Tilde{\mathcal{D}}^k_c,\Tilde{\mathcal{D}}^k_n\}$

\textcolor{blue}{//Section.~\ref{sec:label_est}: soft label estimation by bidirectional cross-modal similarity consistency}

Keep the labels in $\mathcal{B}_j^c$, estimate soft correspondence labels $y^*$ for the noisy data $\mathcal{B}_j^n$ using Eq.~\ref{eq:soft_label}

\textcolor{blue}{//Section.~\ref{sec:soft_loss}: optimize the soft matching loss on the estimated soft correspondence label }

Train the network $k$ on $\{\mathcal{B}_j^c = (I_c,T_c,y_c=1), \mathcal{B}_j^n= (I_n,T_n,y_n=y^*)\}$ by minimizing Eq.~\ref{eq:soft_loss}
}
}
}

\KwOut{Matching models $(A,B)$}
\caption{The training pipeline of our robust cross-model matching framework.}
% \end{algorithmic}
\label{algo}
\end{algorithm*}


